Partially Typed Multiparty Sessions

A multiparty session formalises a set of concurrent communicating participants. We propose a type system for multiparty sessions where some communications between participants can be ignored. This allows us to type some sessions with global types representing interesting protocols, which have no type in the standard type systems. Our type system enjoys Subject Reduction, Session Fidelity and "partial" Lock-freedom. The last property ensures the absence of locks for participants with non ignored communications. A sound and complete type inference algorithm is also discussed.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{C. Aubert, C. Di Giusto, S. Fowler \& L. Safina (Eds.):\\
16th Interaction and Concurrency Experience (ICE 2023)\\
EPTCS 383, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.383.2}{10.4204/EPTCS.383.2}}

